HandOccNet: Occlusion-Robust 3D Hand Mesh Estimation Network

Hands are often severely occluded by objects, which makes 3D hand mesh estimation challenging. Previous works often have disregarded information at occluded regions. However, we argue that occluded regions have strong correlations with hands so that they can provide highly beneficial information for complete 3D hand mesh estimation. Thus, in this work, we propose a novel 3D hand mesh estimation network HandOccNet, that can fully exploits the information at occluded regions as a secondary means to enhance image features and make it much richer. To this end, we design two successive Transformer-based modules, called feature injecting transformer (FIT) and self- enhancing transformer (SET). FIT injects hand information into occluded region by considering their correlation. SET refines the output of FIT by using a self-attention mechanism. By injecting the hand information to the occluded region, our HandOccNet reaches the state-of-the-art performance on 3D hand mesh benchmarks that contain challenging hand-object occlusions. The codes are available in: https://github.com/namepllet/HandOccNet.

==> sections/figures/interesting.tex <==
\begin{figure*}[t]
    \renewcommand{\wp}{0.195\linewidth}
    \subfloat[Input]{\includegraphics[width=\wp]{figure/interesting/2420_img.png}}
    \hfill
    \subfloat[Hasson~\etal~\cite{hasson2020leveraging}]{\includegraphics[width=\wp]{figure/interesting/2420_photo.png}}
    \hfill
    \subfloat[I2L-MeshNet~\cite{moon2020i2l}]{\includegraphics[width=\wp]{figure/interesting/2420_I2L.png}}
    \hfill
    \subfloat[Liu~\etal~\cite{liu2021semi}]{\includegraphics[width=\wp]{figure/interesting/2420_Semi.png}}
    \hfill
    \subfloat[Ours]{\includegraphics[width=\wp]{figure/interesting/2420_ours.png}}
    \figcspace
    \vspace{-5mm}
    \caption{
        Interesting Figures
    }
    \label{fig:interesting}
    \vspace{3mm}
    \figspace
\end{figure*}

==> sections/figures/transformers.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{.6\linewidth}
        \centering
        \includegraphics[width=0.8\linewidth, height=0.3\textheight]{figure/FIN.pdf}
        \caption{FIN}
        \label{fig:FIN}
    \end{minipage}%
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=1.\linewidth, height=0.3\textheight]{figure/FIS.pdf}
        \caption{FIS}
        \label{fig:transformers}
    \end{minipage}
\end{figure}

==> sections/table/crossdomain.tex <==
\begin{table}[t]
    \tabcspace
    \centering
    \vspace{-5mm}
    \begin{tabular}{c|cc|cc}
        \toprule
        \multirow{2}{*}{methods} &
        \multicolumn{2}{c|}{H2F} &
        \multicolumn{2}{c}{F2H} \\
        & joint & mesh & joint & mesh\\
        \midrule
        Hassons~\etal & - & - & - & -\\
        Hampali~\etal & - & - & - & -\\
        Liu~\etal & - & - & - & -\\
        pose2mesh & - & - & - & -\\
        I2L & - & - & - & -\\
        \textbf{HandOCCNet} & - & - & - & -\\
        \bottomrule
    \end{tabular}
    \caption{The quantitative comparison on cross domain validation. H2F denotes trained on HO-3D dataset and evaluated on FPHA dataset. Conversely, F2H denotes trained on FPHA dataset and evaluated on HO-3D dataset.}
    \label{tab:crossdomain}
    \tabspace
    \vspace{3mm}
\end{table}

==> sections/table/ho3d_split.tex <==
\begin{table}[t]
    \newcommand{\cmark}{\ding{51}}%
    \newcommand{\xmark}{\ding{55}}%
    \tabcspace
    \centering
    \begin{tabular}{c|c}
        \toprule
        Methods & 3D joint error \\
        \midrule
        Pose2Mesh~\cite{choi2020pose2mesh} & 14.3\\
        Hasson~\etal~\cite{hasson2020leveraging} & 12.1 \\
        Liu~\etal~\cite{liu2021semi} & 11.3 \\
        I2L-MeshNet~\cite{moon2020i2l} & 11.3\\
        \textbf{HandOccNet (Ours)} & \textbf{9.3}\\
        \bottomrule
    \end{tabular}
    \caption{Comparison with state-of-the-art methods on the selected sequences of HO-3D~(MPM13 and AP12).}
    \label{tab:ho3d-split}
    \tabspace
    \vspace{3mm}
\end{table}

==> supple/fit.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
        \toprule
        Input & Output &  layer & kernel & stride & output shape\\
        \midrule
        $\mathbf{F}_{\text{S}}$ & - & - & - & - & $256 \times 32 \times 32$ \\
        $\mathbf{F}_{\text{P}}$ & - & - & - & - & $256 \times 32 \times 32$ \\
        \midrule
        $q_{\text{soft}}$ & $\mathbf{F}_{\text{S}}$ & conv & $1 \times 1$ & 1 & $256 \times 32 \times 32$\\
        $q_{\text{sig}}$ & $\mathbf{F}_{\text{S}}$ & conv & $1 \times 1$ & 1 & $256 \times 32 \times 32$\\
        $k_{\text{soft}}$ & $\mathbf{F}_{\text{P}}$ & conv & $1 \times 1$ & 1 & $256 \times 32 \times 32$\\
        $k_{\text{sig}}$ & $\mathbf{F}_{\text{P}}$ & conv & $1 \times 1$ & 1 & $256 \times 32 \times 32$\\
        $k_{\text{sig}}$ & $\mathbf{F}_{\text{P}}$ & conv & $1 \times 1$ & 1 & $256 \times 32 \times 32$\\
        $v$ & $\mathbf{F}_{\text{P}}$ & conv & $1 \times 1$ & 1 & $256 \times 32 \times 32$\\
        \midrule
        $q_{\text{soft}}$ & $q_{\text{soft}}$ & reshape & - & - & $32*32  \times 256$\\
        $q_{\text{sig}}$ & $q_{\text{sig}}$ & reshape & - & - & $32*32  \times 256$\\
        $k_{\text{soft}}$ & $k_{\text{soft}}$ & reshape & - & - & $32*32  \times 256$\\
        $k_{\text{sig}}$ & $k_{\text{sig}}$ & reshape & - & - & $32*32  \times 256$\\
        $k_{\text{sig}}$ & $k_{\text{sig}}$ & reshape & - & - & $32*32  \times 256$\\
        $v$ & $v$ & reshape & - & - & $32*32  \times 256$\\
        \midrule
        $q_{\text{soft}}$ $\And$ $k_{\text{soft}}$ & - & Matrix mult. & - & - & $32*32 \times 32*32$\\
        - & $\mathbf{C}_{\text{soft}}$ & softmax & - & - & $32*32 \times 32*32$\\
        \midrule
        $q_{\text{sig}}$ $\And$ $k_{\text{sig}}$ & - & Matrix mult. & - & - & $32*32 \times 32*32$\\
        - & - & average pooling & - & - & $32*32 \times 1$\\
        - & - & FC & - & - & $32*32 \times 1$\\
        - & $\mathbf{C}_{\text{sig}}$ & sigmoid & - & - & $32*32 \times 1$\\
        \midrule
        $\mathbf{C}_{\text{soft}}$ $\And$ $\mathbf{C}_{\text{sig}}$ & $\mathbf{C}$ & Element mult. & - & - & $32*32 \times 32*32$\\
        \midrule
        $\mathbf{C}_{\text{soft}}$ $\And$ $v$ & $\mathbf{R}_{\text{FIT}}$ & Matrix mult. & - & - & $32*32 \times 256$\\
        \midrule
        $\mathbf{R}_{\text{FIT}}$ & - & FC & - & - & $32*32 \times 256$\\
        - & - & ReLU & - & - & $32*32 \times 256$\\
        - & - & FC & - & - & $32*32 \times 256$\\
        - & - & Dropout & - & - & $32*32 \times 256$\\
        - & - & Connections & - & - & $32*32 \times 256$\\
        - & $\mathbf{F}_{\text{FIT}}$ & reshape & - & - & $256 \times 32 \times 32$\\
        \bottomrule
    \end{tabular}
    \tabcspace
    \caption{FIT architecture details.}
    \label{sup_tab:fit}
    \tabcspace
\end{table*}


==> supple/model_figure.tex <==
\begin{figure}[t]
    \centering
    \renewcommand{\wp}{0.45\linewidth}
    \newcommand{\hp}{\hspace{0.1\linewidth}}
    \newcommand{\hhp}{\hspace{0.05\linewidth}}
    \subfloat[The overall architecure of HandOccNet, which consists of backbone, FIT, SET, and regressor.\label{sup_fig:model}]{
    \includegraphics[width=0.98\linewidth]{latex/figure/model.pdf}
    }
    \\
    \vspace{3mm}
    \subfloat[The overall pipeline of FIT. \label{sup_fig:fit}]{
    \includegraphics[height=0.22\linewidth]{latex/figure/FIN.pdf}
    }
    \hhp
    \subfloat[The overall pipeline of SET. \label{sup_fig:set}]{
    \includegraphics[height=0.22\linewidth]{latex/figure/FIS.pdf}
    }
    \figcspace
    \caption{\textbf{Overall architecture and components of our HandOccNet.}}
    \label{fig:model}
    \figspace
\end{figure}

